LiDAR-based 4D Panoptic Segmentation via Dynamic Shifting Network

With the rapid advances of autonomous driving, it becomes critical to equip its sensing system with more holistic 3D perception. However, existing works focus on parsing either the objects (e.g. cars and pedestrians) or scenes (e.g. trees and buildings) from the LiDAR sensor. In this work, we address the task of LiDAR-based panoptic segmentation, which aims to parse both objects and scenes in a unified manner. As one of the first endeavors towards this new challenging task, we propose the Dynamic Shifting Network (DS-Net), which serves as an effective panoptic segmentation framework in the point cloud realm. In particular, DS-Net has three appealing properties: 1) Strong backbone design. DS-Net adopts the cylinder convolution that is specifically designed for LiDAR point clouds. 2) Dynamic Shifting for complex point distributions. We observe that commonly-used clustering algorithms are incapable of handling complex autonomous driving scenes with non-uniform point cloud distributions and varying instance sizes. Thus, we present an efficient learnable clustering module, dynamic shifting, which adapts kernel functions on the fly for different instances. 3) Extension to 4D prediction. Furthermore, we extend DS-Net to 4D panoptic LiDAR segmentation by the temporally unified instance clustering on aligned LiDAR frames. To comprehensively evaluate the performance of LiDAR-based panoptic segmentation, we construct and curate benchmarks from two large-scale autonomous driving LiDAR datasets, SemanticKITTI and nuScenes. Extensive experiments demonstrate that our proposed DS-Net achieves superior accuracies over current state-of-the-art methods in both tasks. Notably, in the single frame version of the task, we outperform the SOTA method by 1.8% in terms of the PQ metric. In the 4D version of the task, we surpass 2nd place by 5.4% in terms of the LSTQ metric.

==> chaps/pics/03_01_baseline_arch.tex <==
% \setcounter{figure}{1}
\begin{figure*}[t]
    \begin{center}
        % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
        \includegraphics[width=1.0\linewidth]{assets/baseline_arch_2.pdf}
    \end{center}
    \caption{\textbf{Architecture of the Strong Backbone.} The backbone consists of a cylinder backbone, a semantic and a instance branch. The backbone provides grid-level features for semantic branch to predict point-wise semantic label which then provides \stuff{} points masks for instance branch to further extract their instance IDs through heuristic clustering algorithms.}
    \label{fig:03_01_baseline_arch}
\end{figure*}

==> chaps/pics/03_02_density_count.tex <==
\begin{figure}[t]
    \begin{center}
        % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
        \includegraphics[width=0.9\linewidth]{assets/density_count.pdf}
    \end{center}
    \caption{\textbf{Density Distribution of the Regressed Centers of the LiDAR Point Clouds.} (a) counts the average number of regressed centers inside each valid voxel of instances at different distances. (b) presents the average number of points of instances at different distances.}
    \label{fig:03_02_density_count}
\end{figure}

==> chaps/pics/03_02_rq_vs_bandwidth.tex <==
\begin{figure}[ht]
    \begin{center}
        % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
        \includegraphics[width=1.0\linewidth]{assets/rq_vs_bandwidth.pdf}
    \end{center}
    \caption{\textbf{Effect of Different Mean Shift Bandwidth on the Recognition Quality of Different Classes.} The Recognition Quality is defined as $\text{TP} / (\text{TP} + 0.5\text{FP} + 0.5\text{FN})$, where $\text{TP}$ means the number of true positives, $\text{FP}$ stands for the number of false positives and $\text{FN}$ represents the number of false negatives. The above metrics are counted using the IoU threshold of $0.5$.}
    \label{fig:03_02_rq_vs_bandwidth}
\end{figure}

==> chaps/pics/03_03_nickname_arch.tex <==
\begin{figure*}[t]
    \begin{center}
        % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
        \includegraphics[width=1.0\linewidth]{assets/learnable_meanshift_arch_2.pdf}
    \end{center}
    \caption{\textbf{Architecture of the \nickname{}.} The \nickname{} takes point-wise features, regressed centers and XYZ coordinates of \things{} classes as input. After a fixed number of MeanShift iterations where the kernel function of each point is dynamically adapted, the points are further clustered and the instance IDs are obtained.}
    \label{fig:03_03_nickname_arch}
\end{figure*}

==> chaps/pics/04_02_demo.tex <==
\begin{figure*}[t]
    \begin{center}
        \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \end{center}
    \caption{This will be the demo on SemanticKITTI.}
    \label{fig:04_02_demo}
\end{figure*}

==> chaps/pics/supp_colab.tex <==
\begin{figure*}[t]
    \begin{center}
        \includegraphics[width=1.0\linewidth]{assets/colab-2020-11-16.png}
    \end{center}
    \caption{Screenshot of the public leaderboard (\url{https://competitions.codalab.org/competitions/24025}) of SemanticKITTI at 2020-11-16. Our method achieves 1st place.}
    \label{fig:supp_colab}
\end{figure*}

==> chaps/tabs/04_02_tab_ab_iter.tex <==
\begin{table}[h]
    \caption{Experiments on the number of iteration. All results in [\%].}
    \begin{center}
    \small{
        \begin{tabular}{c|cccc|c}
            \Xhline{1pt}
            \makecell{Number of\\ Iteration} & \PQ & \PQda & \RQ & \SQ & \miou \\
            \hline\hline
            1 & 57.0          & 62.6          & 67.4          & 77.3          & 63.5          \\
            2 & 57.6          & 63.1          & 67.8          & 77.5          & \textbf{63.6} \\
            3 & \textbf{57.7} & 63.3          & \textbf{68.0} & \textbf{77.6} & 63.4          \\
            4 & \textbf{57.7} & \textbf{63.4} & \textbf{68.0} & \textbf{77.6} & 63.5          \\
            5 & 57.5          & 63.2          & 67.7          & \textbf{77.6} & 63.4          \\
            \Xhline{1pt}
        \end{tabular}
    }
    \end{center}
    \label{tab:ab_iter}
\end{table}



==> chaps/tabs/04_02_tab_ab_reg.tex <==
\begin{table}[h]
    \begin{center}
    \small{
        \begin{tabular}{l|cccc|c}
            \Xhline{1pt}
            Method & \PQ & \PQda & \RQ & \SQ & \miou \\
            \hline\hline
            Direct Regression & 52.0          & 57.6          & 63.1          & 73.9          & \textbf{63.5} \\
            Learning Weights  & \textbf{57.7} & \textbf{63.4} & \textbf{68.0} & \textbf{77.6} & \textbf{63.5} \\
            \Xhline{1pt}
        \end{tabular}
    }
    \end{center}
    \caption{Ablation study on bandwidth learning method. All results in [\%].}
    \label{tab:ab_reg}
\end{table}


==> chaps/tabs/04_02_tab_ab_share.tex <==
\begin{table}[h]
    \begin{center}
    \small{
        \begin{tabular}{l|cccc|c}
            \Xhline{1pt}
            Method & \PQ & \PQda & \RQ & \SQ & \miou \\
            \hline\hline
            Sharing Weights     & \textbf{57.7} & 63.3          & 67.9          & \textbf{77.8} & 63.3          \\
            Not Sharing Weights & \textbf{57.7} & \textbf{63.4} & \textbf{68.0} & 77.6          & \textbf{63.5} \\
            \Xhline{1pt}
        \end{tabular}
    }
    \end{center}
    \caption{Ablation study on weights sharing of bandwidth weights regression. All results in [\%].}
    \label{tab:ab_share}
\end{table}


==> chaps/tabs/04_02_tab_semkitti_pq_per_class.tex <==
\begin{table*}
    \caption{Detailed per-class \PQ{} results on the test set of SemanticKITTI. All results in [\%].}
    \begin{center}
    \tabcolsep=0.13cm
    \scriptsize{
        \begin{tabular}{l|c|ccccccccccccccccccc}
            \Xhline{1pt}
                           
            Method & \PQ & \car  & \truc & \bcle & \mcle & \oveh & \pers & \bcli & \mcli & \road & \side & \park & \ogro & \buil & \vege & \trun & \terr & \fenc & \pole & \traf \\
            \hline\hline
            KPConv\cite{thomas2019kpconv} +
            PointPillars\cite{lang2019pointpillars} & 44.5 & 72.5 & 17.2 &  9.2 & 30.8 & 19.6 & 29.9 & 59.4 & 22.8 & 84.6 & 60.1 & 34.1 & \textbf{8.8} & 80.7 & 77.6 & 53.9 & 42.2 & 49.0 & 46.2 & 46.8 \\
            RangeNet++\cite{milioto2019rangenet++} +
            PointPillars\cite{lang2019pointpillars} & 37.1 & 66.9 &  6.7 &  3.1 & 16.2 &  8.8 & 14.6 & 31.8 & 13.5 & \textbf{90.6} & 63.2 & \textbf{41.3} &  6.7 & 79.2 & 71.2 & 34.6 & 37.4 & 38.2 & 32.8 & 47.4 \\
            KPConv\cite{thomas2019kpconv} +
            PV-RCNN\cite{shi2020pv}                 & 50.2 & 84.5 & 21.9 &  9.9 & 34.2 & 25.6 & 51.1 & 67.9 & 43.8 & 84.9 & \textbf{63.6} & 37.1 &  8.4 & 83.7 & 78.3 & 57.5 & 42.3 & \textbf{51.1} & 51.0 & 57.4 \\
            \hline
            PolarNet\_seg$^{\ast}$                  & 53.3 & 88.7 & \textbf{31.7} & 34.6 & \textbf{50.9} & \textbf{39.1} & 57.5 & 68.7 & 45.1 & 88.1 & 59.7 & 40.5 &  1.0 & \textbf{85.7} & 77.7 & 53.2 & 39.7 & 44.8 & 48.6 & 57.6 \\
            \hline
            Backbone with Fusion                    & 53.1 & 90.6 & 15.8 & 44.2 & 46.9 & 28.5 & 63.1 & 67.7 & 47.6 & 88.2 & 59.4 & 29.5 &  3.0 & 82.5 & 79.0 & 56.6 & 42.3 & 48.1 & 53.2 & 63.6\\
            \nickname{}                             & \textbf{55.9} & \textbf{91.2} & 28.8 & \textbf{45.4} & 47.2 & 34.6 & \textbf{63.6} & \textbf{71.1} & \textbf{58.5} & 89.1 & 61.2 & 32.3 &  4.0 & 83.2 & \textbf{79.6} & \textbf{58.3} & \textbf{43.4} & 50.0 & \textbf{55.2} & \textbf{65.3} \\
            \Xhline{1pt}
        \end{tabular}
    }
    \end{center}
    \label{tab:semkitti_test_pq}
\end{table*}

==> chaps/tabs/04_02_tab_semkitti_rq_per_class.tex <==
\begin{table*}
    \caption{Detailed per-class \RQ{} results on the test set of SemanticKITTI. All results in [\%].}
    \begin{center}
    \tabcolsep=0.13cm
    \scriptsize{
        \begin{tabular}{l|c|ccccccccccccccccccc}
            \Xhline{1pt}
                           
            Method & \RQ & \car  & \truc & \bcle & \mcle & \oveh & \pers & \bcli & \mcli & \road & \side & \park & \ogro & \buil & \vege & \trun & \terr & \fenc & \pole & \traf \\
            \hline\hline
            KPConv\cite{thomas2019kpconv} +
            PV-RCNN\cite{shi2020pv}                 & 61.4 & 94.5 & 26.9 & 14.5 & 43.6 & 32.0 & 70.0 & 76.8 & 52.6 & 91.5 & \textbf{78.7} & 47.7 & \textbf{11.4} & 90.2 & 94.1 & 76.4 & 56.5 & \textbf{66.8} & 68.8 & 74.1 \\
            \hline
            PolarNet\_seg$^{\ast}$                  & 64.2 & 96.2 & \textbf{36.0} & 48.5 & \textbf{58.6} & \textbf{43.0} & 66.2 & 77.1 & 50.3 & 96.3 & 74.8 & \textbf{54.2} &  1.7 & \textbf{92.1} & 94.1 & 72.6 & 53.9 & 61.1 & 66.0 & 76.3 \\
            \hline
            Backbone with Fusion                    & 64.5 & 97.4 & 20.5 & 61.1 & 57.2 & 33.2 & 74.0 & 75.6 & 57.8 & 96.2 & 75.1 & 39.2 & 5.0 & 88.8 & 95.5 & 75.8 & 57.1 & 63.8 & 72.2 & 80.4 \\
            \nickname{}                             & \textbf{66.7} & \textbf{97.5} & 32.4 & \textbf{62.2} & 56.3 & 38.9 & \textbf{74.3} & \textbf{78.4} & \textbf{62.7} & \textbf{96.8} & 76.7 & 42.6 & 6.4 & 89.3 & \textbf{95.7} & \textbf{77.5} & \textbf{58.3} & 65.5 & \textbf{74.0} & \textbf{81.9} \\
            \Xhline{1pt}
        \end{tabular}
    }
    \end{center}
    \label{tab:semkitti_test_rq}
\end{table*}

==> chaps/tabs/04_02_tab_semkitti_sq_per_class.tex <==
\begin{table*}
    \caption{Detailed per-class \SQ{} results on the test set of SemanticKITTI. All results in [\%].}
    \begin{center}
    \tabcolsep=0.13cm
    \scriptsize{
        \begin{tabular}{l|c|ccccccccccccccccccc}
            \Xhline{1pt}
                           
            Method & \SQ & \car  & \truc & \bcle & \mcle & \oveh & \pers & \bcli & \mcli & \road & \side & \park & \ogro & \buil & \vege & \trun & \terr & \fenc & \pole & \traf \\
            \hline\hline
            KPConv\cite{thomas2019kpconv} +
            PV-RCNN\cite{shi2020pv}                 & 80.0 & 89.4 & 81.3 & 68.1 & 78.4 & 79.8 & 73.0 & 88.4 & 83.3 & \textbf{92.9} & \textbf{80.8} & \textbf{77.8} & \textbf{73.4} & 92.8 & \textbf{83.2} & \textbf{75.2} & \textbf{75.0} & \textbf{76.5} & 74.2 & 77.5 \\
            \hline
            PolarNet\_seg$^{\ast}$                  & 81.1 & 92.2 & 88.0 & 71.4 & \textbf{86.9} & \textbf{90.8} & \textbf{87.0} & 89.1 & 89.8 & 91.4 & 79.9 & 74.8 & 55.4 & 93.1 & 82.6 & 73.3 & 73.8 & 73.2 & 73.6 & 75.5 \\
            \hline
            Backbone with Fusion                    & 80.3 & 93.0 & 77.0 & 72.3 & 81.9 & 85.8 & 85.3 & 89.5 & 82.5 & 91.8 & 79.1 & 75.1 & 60.2 & 92.9 & 82.7 & 74.7 & 74.0 & 75.5 & 73.6 & 79.1 \\
            \nickname{}                             & \textbf{82.3} & \textbf{93.6} & \textbf{88.9} & \textbf{73.0} & 83.8 & 89.0 & 85.6 & \textbf{90.7} & \textbf{93.3} & 92.0 & 79.8 & 75.8 & 61.4 & \textbf{93.2} & \textbf{83.2} & \textbf{75.2} & 74.4 & 76.3 & \textbf{74.5} & \textbf{79.7} \\
            \Xhline{1pt}
        \end{tabular}
    }
    \end{center}
    \label{tab:semkitti_test_sq}
\end{table*}
